Learning to Code on Graphs for Topological Interference Management

The state-of-the-art coding schemes for topological interference management (TIM) problems are usually handcrafted for specific families of network topologies, relying critically on experts' domain knowledge. This inevitably restricts the potential wider applications to wireless communication systems, due to the limited generalizability. This work makes the first attempt to advocate a novel intelligent coding approach to mimic topological interference alignment (IA) via local graph coloring algorithms, leveraging the new advances of graph neural networks (GNNs) and reinforcement learning (RL). The proposed LCG framework is then generalized to discover new IA coding schemes, including one-to-one vector IA and subspace IA. The extensive experiments demonstrate the excellent generalizability and transferability of the proposed approach, where the parameterized GNNs trained by small size TIM instances are able to work well on new unseen network topologies with larger size.

==> Learning to Code on Graphs for Topological Interference Management (journal) (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
% my def
\def\cleanup{\textit{clean-up}}
\def\cleanone{\textit{clean-up-\uppercase\expandafter{\romannumeral1}}}
\def\cleantwo{\textit{clean-up-\uppercase\expandafter{\romannumeral2}}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution


\newcommand{\Ls}{\mathcal{L}}

\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Learning to Code on Graphs for Topological Interference Management (journal) (1)/typeset_equations_v4.6/dot_emacs <==
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;;; Copyright Stefan M. Moser
;;; 
;;; Version 1.0, 17 September 2004
;;; Version 1.1, 28 October 2004: changed IEEEeqnarray
;;; Version 2.0, 4 June 2006: improved IEEEeqnarray, linebreak, IEEEmulticol; 
;;;              added IEEEeqnarraystar
;;; Version 2.1, 30 March 2007: added linebreakwithoutspace, small corrections
;;; Version 3.0, 13 October 2008: removed \C-s and replaced by secure version 
;;;              that is independent of keyboard definitions
;;; Version 3.3, 29 March 2011: added \IEEElabel
;;; Version 3.5, 29 October 2011: worked over
;;; Version 4.0, 3 January 2013: removed IEEElabel
;;; Version 4.2, 6 August 2013: replace \: with \>
;;; Version 4.6, 29 September 2017: added \IEEEeqnarraylabel, \subnumberinglabel,
;;;              \IEEElabelanchoreqn
;;;
;;; You may change this code, but you always have to keep this 
;;; header (you may add to it).
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;

;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add somewhere in your .emacs-file:

(fset 'IEEEeqnarray
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} tab up tab])

(fset 'IEEEeqnarraystar
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} tab up tab])

(fset 'linebreak
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right ?\\ ?> tab])

(fset 'linebreakwithoutspace
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right tab])

(fset 'unlinebreak
   [?\C-\M-s ?\\ ?n ?o ?n ?u ?m ?b ?e ?r C-left left ?\C-  ?\C-\M-s ?& ?& right left ?\C-w])

(fset 'IEEEmulticol
   [?\C-a tab ?\\ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?m ?u ?l ?t ?i ?c ?o ?l ?{ ?3 ?} ?{ ?l ?} ?{ return tab escape ?x ?i ?s ?e ?a ?r ?c ?h ?- ?f ?o ?r ?w ?a ?r ?d return ?& left ?} ?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ ?\\ ?q ?u ?a ?d return tab])


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add the eight marked lines in the LaTeX-mode-hook, or if not 
;; existent, copy whole paragraph into your .emacs-file:
(require 'tex-site)
(setq LaTeX-mode-hook 
 '(lambda ()
    (define-key LaTeX-mode-map "\C-ci" 'IEEEeqnarray)         ;; add this line!
    (define-key LaTeX-mode-map "\C-co" 'IEEEeqnarraystar)     ;; add this line!
    (define-key LaTeX-mode-map "\C-cb" 'linebreak)            ;; add this line!
    (define-key LaTeX-mode-map "\C-cn" 'linebreakwithoutspace);; add this line!
    (define-key LaTeX-mode-map "\C-c\C-b" 'unlinebreak)       ;; add this line!
    (define-key LaTeX-mode-map "\C-cm" 'IEEEmulticol)         ;; add this line!
    (auto-fill-mode)
    (turn-on-reftex)
    (setq LaTeX-environment-list 
	  '(
	    (("abstract"))
	    (("array" LaTeX-env-array))
	    (("cases"))
	    (("center"))
	    (("claim" LaTeX-env-label))
	    (("conjecture" LaTeX-env-label))
	    (("corollary" LaTeX-env-label))
	    (("definition" LaTeX-env-label))
	    (("description" LaTeX-env-item))
	    (("document" LaTeX-env-document))
	    (("enumerate" LaTeX-env-item))
	    (("equation" LaTeX-env-label))
	    (("equation*"))
	    (("IEEEeqnarray" LaTeX-env-label))    ;; add this line!
	    (("IEEEeqnarray*"))                   ;; add this line!
	    (("example" LaTeX-env-label))
	    (("figure" LaTeX-env-figure))
	    (("figure*" LaTeX-env-figure))
		;(("filecontents" LaTeX-env-contents))
		;(("filecontents*" LaTeX-env-contents))
		;(("flushleft"))
		;(("flushright"))
	    (("itemize" LaTeX-env-item))
	    (("lemma" LaTeX-env-label))
	    (("list" LaTeX-env-list))
	    (("minipage" LaTeX-env-minipage))
	    (("multline" LaTeX-env-label))
	    (("multline*"))
	    (("picture" LaTeX-env-picture))
	    (("proposition" LaTeX-env-label))
	    (("quotation"))
	    (("quote"))
	    (("remark" LaTeX-env-label))
	    (("sloppypar"))
	    (("tabbing"))
	    (("table" LaTeX-env-figure))
	    (("table*" LaTeX-env-figure))
	    (("tabular" LaTeX-env-array))
	    (("tabular*" LaTeX-env-tabular*))
	    (("thebibliography" LaTeX-env-bib))
	    (("theindex" LaTeX-env-item))
	    (("theorem" LaTeX-env-label))
	    (("titlepage"))
	    (("trivlist" LaTeX-env-item))
	    (("verbatim"))
	    (("verbatim*"))
	    (("verse"))
	    )
	  )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarry/IEEEeqnarraybox known to
;; ispell: the spelling tool of Emacs.
;; Add the three marked lines to the ispell-tex-skip-alists in the corresponding
;; position, or if not existent, copy whole paragraph into your .emacs-file:
(setq ispell-local-dictionary "american")
(add-hook 'tex-mode-hook (function (lambda () (setq ispell-parser 'tex))))
(require 'ispell)
(setq ispell-tex-skip-alists
  '((
     ("%\\[" . "%\\]")
     ;; All the standard LaTeX keywords from L. Lamport's guide:
     ;; \cite, \hspace, \hspace*, \hyphenation, \include, \includeonly, \input,
     ;; \label, \nocite, \rule (in ispell - rest included here)
     ("\\\\addcontentsline"              ispell-tex-arg-end 2)
     ("\\\\psfrag"                       ispell-tex-arg-end-psfrag 0)
     ("\\\\add\\(tocontents\\|vspace\\)" ispell-tex-arg-end)
     ("\\\\\\([aA]lph\\|arabic\\)"       ispell-tex-arg-end)
     ("\\\\author"                       ispell-tex-arg-end)
     ("\\\\bibliographystyle"            ispell-tex-arg-end)
     ("\\\\bibliography"                 ispell-tex-arg-end)
     ("\\\\bstctlcite"                   ispell-tex-arg-end)
     ("\\\\eqref"                        ispell-tex-arg-end)
     ("\\\\thref"                        ispell-tex-arg-end)
     ("\\\\label"                        ispell-tex-arg-end)
     ("\\\\makebox"                      ispell-tex-arg-end 0)
     ("\\\\document\\(class\\|style\\)" .
      "\\\\begin[ \t\n]*{[ \t\n]*document[ \t\n]*}")
     )
    (;; delimited with \begin.  In ispell: displaymath, eqnarray, eqnarray*,
     ;; equation, minipage, picture, tabular, tabular* (ispell)
     ("\\(figure\\|table\\)\\*?"  ispell-tex-arg-end 0)
     ("list"                      ispell-tex-arg-end 2)
     ("IEEEeqnarray\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarray\\*?[ \t\n]*}");; add this line!
     ("IEEEeqnarraybox[tm]?\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarraybox[tm]?\\*?[ \t\n]*}");; add this line!
     ("program"         . "\\\\end[ \t\n]*{[ \t\n]*program[ \t\n]*}")
     ("verbatim\\*?"    . "\\\\end[ \t\n]*{[ \t\n]*verbatim\\*?[ \t\n]*}")
     ("gather\\*?"      . "\\\\end[ \t\n]*{[ \t\n]*gather\\*?[ \t\n]*}")
     )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarray known to reftex: the referencing 
;; tool of Emacs.  
;; Add the three marked lines to your reftex-label-alist, or if not
;; existent, copy whole paragraph into your .emacs-file:
(setq reftex-label-alist
 '(
   (nil              ?e "eq:"   "~\\eqref{%s}" nil nil)
   ("IEEEeqnarray"   ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("IEEEeqnarray*"  ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("\\IEEEeqnarraylabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\subnumberinglabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\IEEElabelanchoreqn{*}"     ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("lemma"          ?l "lem:"  "~\\ref{%s}"   t   ("lemma" "lem."))
   ("theorem"        ?h "thm:"  "~\\ref{%s}"   t   ("theorem" "th." "thm."))  
   ("corollary"      ?c "cor:"  "~\\ref{%s}"   t   ("corollary" "cor."))  
   ("conjecture"     ?j "conj:" "~\\ref{%s}"   t   ("conjecture" "conj."))  
   ("proposition"    ?p "prop:" "~\\ref{%s}"   t   ("proposition" "prop."))  
   ("claim"          ?m "clm:"  "~\\ref{%s}"   t   ("claim" "cl."))  
   ("definition"     ?d "def:"  "~\\ref{%s}"   t   ("definition" "def."))  
   ("remark"         ?r "rem:"  "~\\ref{%s}"   t   ("remark" "rem."))  
   ("example"        ?x "ex:"   "~\\ref{%s}"   t   ("example" "ex."))  
   ("exercise"       ?x "ex:"   "~\\ref{%s}"   t   ("exercise" "exer." "exerc." "ex."))  
   ("enumerate"      ?i "item:" "~\\ref{%s}"   t   ("part"))  
   ))



==> typeset_equations_v4.6/dot_emacs <==
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;;; Copyright Stefan M. Moser
;;; 
;;; Version 1.0, 17 September 2004
;;; Version 1.1, 28 October 2004: changed IEEEeqnarray
;;; Version 2.0, 4 June 2006: improved IEEEeqnarray, linebreak, IEEEmulticol; 
;;;              added IEEEeqnarraystar
;;; Version 2.1, 30 March 2007: added linebreakwithoutspace, small corrections
;;; Version 3.0, 13 October 2008: removed \C-s and replaced by secure version 
;;;              that is independent of keyboard definitions
;;; Version 3.3, 29 March 2011: added \IEEElabel
;;; Version 3.5, 29 October 2011: worked over
;;; Version 4.0, 3 January 2013: removed IEEElabel
;;; Version 4.2, 6 August 2013: replace \: with \>
;;; Version 4.6, 29 September 2017: added \IEEEeqnarraylabel, \subnumberinglabel,
;;;              \IEEElabelanchoreqn
;;;
;;; You may change this code, but you always have to keep this 
;;; header (you may add to it).
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;

;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add somewhere in your .emacs-file:

(fset 'IEEEeqnarray
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} tab up tab])

(fset 'IEEEeqnarraystar
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} tab up tab])

(fset 'linebreak
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right ?\\ ?> tab])

(fset 'linebreakwithoutspace
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right tab])

(fset 'unlinebreak
   [?\C-\M-s ?\\ ?n ?o ?n ?u ?m ?b ?e ?r C-left left ?\C-  ?\C-\M-s ?& ?& right left ?\C-w])

(fset 'IEEEmulticol
   [?\C-a tab ?\\ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?m ?u ?l ?t ?i ?c ?o ?l ?{ ?3 ?} ?{ ?l ?} ?{ return tab escape ?x ?i ?s ?e ?a ?r ?c ?h ?- ?f ?o ?r ?w ?a ?r ?d return ?& left ?} ?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ ?\\ ?q ?u ?a ?d return tab])


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add the eight marked lines in the LaTeX-mode-hook, or if not 
;; existent, copy whole paragraph into your .emacs-file:
(require 'tex-site)
(setq LaTeX-mode-hook 
 '(lambda ()
    (define-key LaTeX-mode-map "\C-ci" 'IEEEeqnarray)         ;; add this line!
    (define-key LaTeX-mode-map "\C-co" 'IEEEeqnarraystar)     ;; add this line!
    (define-key LaTeX-mode-map "\C-cb" 'linebreak)            ;; add this line!
    (define-key LaTeX-mode-map "\C-cn" 'linebreakwithoutspace);; add this line!
    (define-key LaTeX-mode-map "\C-c\C-b" 'unlinebreak)       ;; add this line!
    (define-key LaTeX-mode-map "\C-cm" 'IEEEmulticol)         ;; add this line!
    (auto-fill-mode)
    (turn-on-reftex)
    (setq LaTeX-environment-list 
	  '(
	    (("abstract"))
	    (("array" LaTeX-env-array))
	    (("cases"))
	    (("center"))
	    (("claim" LaTeX-env-label))
	    (("conjecture" LaTeX-env-label))
	    (("corollary" LaTeX-env-label))
	    (("definition" LaTeX-env-label))
	    (("description" LaTeX-env-item))
	    (("document" LaTeX-env-document))
	    (("enumerate" LaTeX-env-item))
	    (("equation" LaTeX-env-label))
	    (("equation*"))
	    (("IEEEeqnarray" LaTeX-env-label))    ;; add this line!
	    (("IEEEeqnarray*"))                   ;; add this line!
	    (("example" LaTeX-env-label))
	    (("figure" LaTeX-env-figure))
	    (("figure*" LaTeX-env-figure))
		;(("filecontents" LaTeX-env-contents))
		;(("filecontents*" LaTeX-env-contents))
		;(("flushleft"))
		;(("flushright"))
	    (("itemize" LaTeX-env-item))
	    (("lemma" LaTeX-env-label))
	    (("list" LaTeX-env-list))
	    (("minipage" LaTeX-env-minipage))
	    (("multline" LaTeX-env-label))
	    (("multline*"))
	    (("picture" LaTeX-env-picture))
	    (("proposition" LaTeX-env-label))
	    (("quotation"))
	    (("quote"))
	    (("remark" LaTeX-env-label))
	    (("sloppypar"))
	    (("tabbing"))
	    (("table" LaTeX-env-figure))
	    (("table*" LaTeX-env-figure))
	    (("tabular" LaTeX-env-array))
	    (("tabular*" LaTeX-env-tabular*))
	    (("thebibliography" LaTeX-env-bib))
	    (("theindex" LaTeX-env-item))
	    (("theorem" LaTeX-env-label))
	    (("titlepage"))
	    (("trivlist" LaTeX-env-item))
	    (("verbatim"))
	    (("verbatim*"))
	    (("verse"))
	    )
	  )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarry/IEEEeqnarraybox known to
;; ispell: the spelling tool of Emacs.
;; Add the three marked lines to the ispell-tex-skip-alists in the corresponding
;; position, or if not existent, copy whole paragraph into your .emacs-file:
(setq ispell-local-dictionary "american")
(add-hook 'tex-mode-hook (function (lambda () (setq ispell-parser 'tex))))
(require 'ispell)
(setq ispell-tex-skip-alists
  '((
     ("%\\[" . "%\\]")
     ;; All the standard LaTeX keywords from L. Lamport's guide:
     ;; \cite, \hspace, \hspace*, \hyphenation, \include, \includeonly, \input,
     ;; \label, \nocite, \rule (in ispell - rest included here)
     ("\\\\addcontentsline"              ispell-tex-arg-end 2)
     ("\\\\psfrag"                       ispell-tex-arg-end-psfrag 0)
     ("\\\\add\\(tocontents\\|vspace\\)" ispell-tex-arg-end)
     ("\\\\\\([aA]lph\\|arabic\\)"       ispell-tex-arg-end)
     ("\\\\author"                       ispell-tex-arg-end)
     ("\\\\bibliographystyle"            ispell-tex-arg-end)
     ("\\\\bibliography"                 ispell-tex-arg-end)
     ("\\\\bstctlcite"                   ispell-tex-arg-end)
     ("\\\\eqref"                        ispell-tex-arg-end)
     ("\\\\thref"                        ispell-tex-arg-end)
     ("\\\\label"                        ispell-tex-arg-end)
     ("\\\\makebox"                      ispell-tex-arg-end 0)
     ("\\\\document\\(class\\|style\\)" .
      "\\\\begin[ \t\n]*{[ \t\n]*document[ \t\n]*}")
     )
    (;; delimited with \begin.  In ispell: displaymath, eqnarray, eqnarray*,
     ;; equation, minipage, picture, tabular, tabular* (ispell)
     ("\\(figure\\|table\\)\\*?"  ispell-tex-arg-end 0)
     ("list"                      ispell-tex-arg-end 2)
     ("IEEEeqnarray\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarray\\*?[ \t\n]*}");; add this line!
     ("IEEEeqnarraybox[tm]?\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarraybox[tm]?\\*?[ \t\n]*}");; add this line!
     ("program"         . "\\\\end[ \t\n]*{[ \t\n]*program[ \t\n]*}")
     ("verbatim\\*?"    . "\\\\end[ \t\n]*{[ \t\n]*verbatim\\*?[ \t\n]*}")
     ("gather\\*?"      . "\\\\end[ \t\n]*{[ \t\n]*gather\\*?[ \t\n]*}")
     )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarray known to reftex: the referencing 
;; tool of Emacs.  
;; Add the three marked lines to your reftex-label-alist, or if not
;; existent, copy whole paragraph into your .emacs-file:
(setq reftex-label-alist
 '(
   (nil              ?e "eq:"   "~\\eqref{%s}" nil nil)
   ("IEEEeqnarray"   ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("IEEEeqnarray*"  ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("\\IEEEeqnarraylabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\subnumberinglabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\IEEElabelanchoreqn{*}"     ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("lemma"          ?l "lem:"  "~\\ref{%s}"   t   ("lemma" "lem."))
   ("theorem"        ?h "thm:"  "~\\ref{%s}"   t   ("theorem" "th." "thm."))  
   ("corollary"      ?c "cor:"  "~\\ref{%s}"   t   ("corollary" "cor."))  
   ("conjecture"     ?j "conj:" "~\\ref{%s}"   t   ("conjecture" "conj."))  
   ("proposition"    ?p "prop:" "~\\ref{%s}"   t   ("proposition" "prop."))  
   ("claim"          ?m "clm:"  "~\\ref{%s}"   t   ("claim" "cl."))  
   ("definition"     ?d "def:"  "~\\ref{%s}"   t   ("definition" "def."))  
   ("remark"         ?r "rem:"  "~\\ref{%s}"   t   ("remark" "rem."))  
   ("example"        ?x "ex:"   "~\\ref{%s}"   t   ("example" "ex."))  
   ("exercise"       ?x "ex:"   "~\\ref{%s}"   t   ("exercise" "exer." "exerc." "ex."))  
   ("enumerate"      ?i "item:" "~\\ref{%s}"   t   ("part"))  
   ))


